PC-SwinMorph: Patch Representation for Unsupervised Medical Image Registration and Segmentation

Medical image registration and segmentation are critical tasks for several clinical procedures. Manual realisation of those tasks is time-consuming and the quality is highly dependent on the level of expertise of the physician. To mitigate that laborious task, automatic tools have been developed where the majority of solutions are supervised techniques. However, in medical domain, the strong assumption of having a well-representative ground truth is far from being realistic. To overcome this challenge, unsupervised techniques have been investigated. However, they are still limited in performance and they fail to produce plausible results. In this work, we propose a novel unified unsupervised framework for image registration and segmentation that we called PC-SwinMorph. The core of our framework is two patch-based strategies, where we demonstrate that patch representation is key for performance gain. We first introduce a patch-based contrastive strategy that enforces locality conditions and richer feature representation. Secondly, we utilise a 3D window/shifted-window multi-head self-attention module as a patch stitching strategy to eliminate artifacts from the patch splitting. We demonstrate, through a set of numerical and visual results, that our technique outperforms current state-of-the-art unsupervised techniques.

==> table/table_1.tex <==

\begin{table*}[th]
\resizebox{1\textwidth}{!}{
\centering
\begin{tabular}{ccccccccccccccccccc}
\hline \toprule[1pt]
{\textsc{Task}} & \textsc{Technique} & {\cellcolor[HTML]{EFEFEF}\textsc{C-WM}} & {\cellcolor[HTML]{EFEFEF}\textsc{C-CX}} & {\cellcolor[HTML]{EFEFEF}\textsc{L-V}} & {\cellcolor[HTML]{EFEFEF}\textsc{L-WM}} & {\cellcolor[HTML]{EFEFEF}\textsc{L-CX}} & {\cellcolor[HTML]{EFEFEF}\textsc{T-P}} & {\cellcolor[HTML]{EFEFEF}\textsc{Cau}} & {\cellcolor[HTML]{EFEFEF}\textsc{Put}} & {\cellcolor[HTML]{EFEFEF}\textsc{Pal}} & {\cellcolor[HTML]{EFEFEF}\textsc{3-V}} & {\cellcolor[HTML]{EFEFEF}\textsc{4-V}} & {\cellcolor[HTML]{EFEFEF}\textsc{B-S}} & {\cellcolor[HTML]{EFEFEF}\textsc{Hipp}} & {\cellcolor[HTML]{EFEFEF}\textsc{Amy}} & {\cellcolor[HTML]{EFEFEF}\textsc{CSF}} & {\cellcolor[HTML]{EFEFEF}\textsc{V-DC}} & {\cellcolor[HTML]{EFEFEF}\textsc{AVG}} \\ \midrule[0.8pt]

\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Registration}}} 
& \textit{VoxelMorph} & 0.777 & 0.829 & 0.791 & 0.682 & 0.815 & 0.849 & 0.795 & 0.804 & 0.734 & 0.644 & 0.733 & 0.881 & 0.654 & 0.659 & 0.611 & 0.790 & 0.753  \\
& \textit{SYMNet} & 0.787 & 0.840 & 0.778 & 0.717 & 0.838 & 0.883 & 0.825 & 0.853 & 0.787 & 0.657 & 0.710 & 0.865 & 0.680 & 0.675 & 0.599 & 0.805 & 0.769 \\
& \textit{DeepTag} & 0.770 & 0.847 & 0.792 & 0.755 & 0.885 & 0.870 & 0.823 & 0.830 & 0.753 & 0.680 & 0.725 & 0.892 & 0.710 & 0.679 & 0.545 & 0.804 & 0.773 \\
& \textit{CycleMorph} & 0.806 & 0.859 & 0.809 & 0.733 & 0.860 & 0.848 & 0.811 & 0.828 & 0.748 & 0.663 & 0.757 & 0.891 & 0.685 & 0.652 & 0.614 & 0.791 & 0.772 \\
& \textbf{\textit{PC-SwinMorph}} & \textbf{0.825} & \textbf{0.880} & \textbf{0.847} & \textbf{0.801} & \textbf{0.908} & \textbf{0.892} & \textbf{0.859} & \textbf{0.880} & \textbf{0.802} & \textbf{0.676} & \textbf{0.784} & \textbf{0.913} & \textbf{0.763} & \textbf{0.698} & \textbf{0.614} & \textbf{0.824} & \textbf{0.812} \\ \midrule[0.8pt]

\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Segmentation}}}
& \textit{VoxelMorph} & 0.776 & 0.831 & 0.783 & 0.698 & 0.812 & 0.860 & 0.802 & 0.830 & 0.764 & 0.673 & 0.738 & 0.881 & 0.663 & 0.669 & 0.574 & 0.797 & 0.759 \\
& \textit{SYMNet} & 0.729 & 0.781 & 0.767 & 0.790 & 0.769 & 0.726 & 0.780 & 0.803 & 0.758 & 0.764 & 0.771 & 0.764 & 0.777 & 0.664 & 0.771 & 0.760 & 0.760 \\
& \textit{DeepTag} & 0.759 & 0.842 & 0.786 & 0.758 & 0.883 & 0.867 & 0.812 & 0.834 & 0.756 & 0.659 & 0.708 & 0.887 & 0.718 & 0.696 & 0.538 & 0.800 & 0.771 \\
& \textit{CycleMorph} & 0.812 & 0.869 & 0.787 & 0.759 & 0.869 & 0.864 & 0.811 & 0.844 & 0.776 & 0.680 & 0.737 & 0.891 & 0.709 & 0.690 & 0.570 & 0.801 & 0.780 \\ 
& \textbf{\textit{PC-SwinMorph}} & \textbf{0.834} & \textbf{0.885} & \textbf{0.847} & \textbf{0.806} & \textbf{0.912} & \textbf{0.888} & \textbf{0.855} & \textbf{0.878} & \textbf{0.802} & \textbf{0.681} & \textbf{0.786} & \textbf{0.915} & \textbf{0.781} & \textbf{0.718} & \textbf{0.610} & \textbf{0.823} & \textbf{0.817} \\ \bottomrule[2pt]
\end{tabular}%
}
\caption{Numerical comparisons between our proposed PC-SwinMorph technique and SOTA techniques on the CANDI dataset. The $Dice$ similarity metric for each region is listed. We denote the regions as C-WM (L/R-Cerebral-WM), C-CX (L/R-Cerebral-CX), L-V (L/R-Lateral-Vent), L-WM (L/R-Cerebellum-WM), L-CX (L/R-Cerebellum-CX), T-P (L/R-Thalamus-Proper), Cau. (L/R-Caudate), Put. (L/R-Putamen), Pal. (L/R-Pallidum), 3-V (3rd-Vent), 4-V (4rd-Vent), CSF, B-S (Brain-Stem), Hipp. (L/R-Hippocampus), Amy. (L/R-Amygdala), V-DC (L/R-VentralDC). The average of the $Dice$ metric over all regions is presented in the last column. The best performance is highlighted in bold font. }
\label{candi_results}
\end{table*}

==> table/table_2.tex <==

\begin{table*}[th]
\centering
\resizebox{0.75\textwidth}{!}{
\begin{tabular}{cccccccccc}
\hline \toprule[1pt]
\textsc{Task} & 
\textsc{Technique} &
 \small \cellcolor[HTML]{EFEFEF} \textsc{Frontal} &
 \small \cellcolor[HTML]{EFEFEF} \textsc{Parietal} & 
 \small \cellcolor[HTML]{EFEFEF} \textsc{Occipital}  & 
 \small \cellcolor[HTML]{EFEFEF} \textsc{Temporal}   & 
 \small \cellcolor[HTML]{EFEFEF} \textsc{Cingulate} & 
 \small \cellcolor[HTML]{EFEFEF} \textsc{Putamen} & 
 \small \cellcolor[HTML]{EFEFEF} \textsc{Hippo} & 
 \small \hspace{0.3cm} \cellcolor[HTML]{EFEFEF} \textsc{AVG} \\ \midrule[0.8pt]
 
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Registration}}} 
 & \textit{VoxelMorph} & 0.866 & 0.709 & 0.683 & 0.797 & 0.679 & 0.648 & 0.654 & \hspace{0.5cm}0.720 \\
 & \textit{SYMNet} & 0.880 & 0.741 & 0.712 & 0.821 & 0.708 & 0.729 & 0.689 & \hspace{0.5cm}0.755 \\
 & \textit{DeepTag} & 0.893 & 0.756 & 0.745 & 0.845 & 0.736 & 0.743 & 0.710 & \hspace{0.5cm}0.775 \\
 & \textit{CycleMorph} & 0.889 & 0.747 & 0.735 & 0.849 & 0.723 & 0.758 & 0.705 & \hspace{0.5cm}0.772 \\
 & \textbf{\textit{PC-SwinMorph }} & \textbf{0.900} & \textbf{0.767} & \textbf{0.751} & \textbf{0.860} & \textbf{0.744} & \textbf{0.780} & \textbf{0.725} & \hspace{0.5cm}\textbf{0.790} \\ \midrule[0.8pt]


 \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Segmentation}}} 
 & \textit{VoxelMorph} & 0.871 & 0.716 & 0.702 & 0.802 & 0.686 & 0.643 & 0.667 & \hspace{0.5cm}0.728    \\ 
 & \textit{SYMNet} & 0.888 & 0.745 & 0.737 & 0.826 & 0.716 & 0.730 & 0.687 & \hspace{0.5cm}0.762 \\
 & \textit{DeepTag} & 0.898 & 0.758 & 0.763 & 0.848 & 0.739 & 0.742 & 0.708 & \hspace{0.5cm}0.780 \\
 & \textit{CycleMorph} & 0.895 & 0.758 & 0.765 & 0.851 & 0.732 & 0.758 & 0.705 & \hspace{0.5cm}0.782 \\ 
 & \textbf{\textit{PC-SwinMorph}} & \textbf{0.901} & \textbf{0.766} & \textbf{0.771} & \textbf{0.860} & \textbf{0.743} & \textbf{0.773} & \textbf{0.729} & \hspace{0.5cm}\textbf{0.794} \\ \bottomrule[2pt]
\end{tabular}
}
\caption{
Numerical comparisons between our proposed PC-SwinMorph technique and SOTA techniques on the LPBA40 dataset. The $Dice$ similarity metric for each region is listed, while the average of the $Dice$ metric over all regions is presented in the last column. The best performance is highlighted in bold font.}
\label{lpba40_results}
\end{table*}
